Canonical Constraints on Leptonic Cp Violation using UHCR neutrino fluxes

It is shown that one can in principle constrain the CP-violating parameter delta from measurements of four independant |V_{ij}|^2, or three of them and a ratio, in the leptonic sector. To quantify our approach, using unitarity, we derive simple expressions in terms of four independant |V_{ij}|^2 for cos(delta) and an expression for sin^2(delta) from J^2. Thus, depending on the values of |V_{ij}| and their accuracy, we can set meaningful limits on |delta|. To illustrate numerically, if |V_{u1}|^2 is close to 0.1 with a 10% precision, and if |V_{e3}^2 is larger than 0.005 and for values of |V_{e2}|^2 and |V_{u3}|^2 that stay within +-0.1 of the current experimental data leads to a bound pi/2 < |delta| < pi. Alternatively, a certain combination of parameters with values of |V_{e3}|^2 larger than 0.01 leads to a closed bound of 73 < |delta| < 103. In general, we find that it is better to use |V_{u1}|^2 or |V_{t1}|^2 as the fourth independant |V_{ij}|^2 and that over most of the parameter space, delta is least sensitive to |V_{e3}|^2. With just three independant measurements (solar, atmospheric and reactor) it is impossible to set limits on the CP phase. In this respect, we study the use of ultra high energy cosmic (UHCR) neutrino fluxes as the additional fourth information. We find that within the SM, neutrino fluxes of all three flavours will be very similar but that pushing current neutrino data to their extreme values still allowed, ratios of cosmic neutrino fluxes can differ by up to 20%; such large discrepancies could imply negligibly small CP-violation. We also study a non radiative neutrino decay model and find that the neutrino fluxes can differ by a factor of up to 3 within this model and that an accuracy of 10% on the neutrino fluxes is sufficient to set interestin limits on delta.

==> paptable1.tex <==
\magnification=1200
\baselineskip=0.25truein
\hsize=16truecm
\vsize=24.5truecm
%\topskip=1.5truecm
\nopagenumbers

%\midinsert
$$\vbox{\offinterlineskip
\halign{&\vrule#&\strut\ #\ \cr
\multispan{15}\hfil\bf Table I \hfil\cr
\hfil\cr
\noalign{\smallskip}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil $|V_{e2}|^2$\hfil&&\hfil $|V_{\mu 3}|^2$\hfil&&\hfil 
$|V_{e3}|^2$\hfil&&\hfil$\rho_1,\rho_2,|V_{\mu 1}|^2$\hfil&&\hfil
$cos(\delta)_-$\hfil&&\hfil $cos(\delta)_c$\hfil&&
\hfil $cos(\delta)_+$\hfil&\cr 
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (10)\hfil&&\hfil 0.50 (10)\hfil&&\hfil 0.03 (10) \hfil&&\hfil
$\rho_1=1.0$ (10)\hfil&&\hfil -0.257\hfil&&
\hfil 0.056\hfil&&\hfil 0.387\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2=2.3$ (10)\hfil&&\hfil -0.300\hfil&&
\hfil 0.111\hfil&&\hfil 0.457\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (10)\hfil&&\hfil -0.708\hfil&&
\hfil -0.132\hfil&&\hfil 0.442\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
$\rho_1=1.0$ (5)\hfil&&\hfil -0.224\hfil&&
\hfil 0.033\hfil&&\hfil 0.294\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2=2.3$ (5)\hfil&&\hfil -0.285\hfil&&
\hfil 0.042\hfil&&\hfil 0.329\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -0.569\hfil&&
\hfil -0.076\hfil&&\hfil 0.414\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (20) \hfil&&\hfil
$\rho_1=1.0$ (5)\hfil&&\hfil -0.247\hfil&&
\hfil 0.033\hfil&&\hfil 0.310\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil     \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$\rho_2=2.3$ (5)\hfil&&\hfil -0.303\hfil&&
\hfil 0.042\hfil&&\hfil 0.343\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -0.607\hfil&&
\hfil -0.076\hfil&&\omit\hfil 0.457\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
$\rho_1 = 1.0$ (10)\hfil&&\hfil -0.306\hfil&&
\hfil 0.033\hfil&&\omit\hfil 0.391\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$\rho_2=2.3$ (10)\hfil&&\hfil -0.404\hfil&&
\hfil 0.042\hfil&&\omit\hfil 0.440\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (10)\hfil&&\hfil -0.747\hfil&&
\hfil -0.076\hfil&&\omit\hfil 0.599\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.015 (5) \hfil&&\hfil
$\rho_1 = 1.0$ (5)\hfil&&\hfil -0.170\hfil&&
\hfil 0.040\hfil&&\omit\hfil 0.255\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$\rho_2=2.3$ (5)\hfil&&\hfil -0.190\hfil&&
\hfil 0.065\hfil&&\omit\hfil 0.300\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -0.493\hfil&&
\hfil -0.093\hfil&&\omit\hfil 0.306\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.005 (5) \hfil&&\hfil
$\rho_1 = 1.0$ (5)\hfil&&\hfil -0.339\hfil&&
\hfil 0.023\hfil&&\omit\hfil 0.392\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 2.3$ (5)\hfil&&\hfil -0.429\hfil&&
\hfil 0.007\hfil&&\omit\hfil 0.412\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -0.756\hfil&&
\hfil -0.054\hfil&&\omit\hfil 0.642\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (2)\hfil&&\hfil 0.001 (25) \hfil&&\hfil
$\rho_1 = 1.0$ (5)\hfil&&\hfil -0.529\hfil&&
\hfil 0.010\hfil&&\omit\hfil 0.555\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 2.3$ (5)\hfil&&\hfil -1.0\hfil&&
\hfil -0.081\hfil&&\omit\hfil 0.885\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -1.0\hfil&&
\hfil -0.024\hfil&&\omit\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (2)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.001 (25) \hfil&&\hfil
$\rho_1 = 1.0$ (5)\hfil&&\hfil -0.879\hfil&&
\hfil 0.010\hfil&&\omit\hfil 0.901\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 2.3$ (5)\hfil&&\hfil -0.796\hfil&&
\hfil -0.081\hfil&&\omit\hfil 0.552\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.15$ (5)\hfil&&\hfil -1.0\hfil&&
\hfil -0.024\hfil&&\omit\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}\noalign{\smallskip}}}
$$
%\endinsert
\noindent
Values of $cos(\delta)$ for different 
combinations of parameters: $cos(\delta)_c$ is obtained  
from the central values of the parameters while $cos(\delta)_-$ and 
$cos(\delta)_+$ are the extremum values allowed by the 
uncertainties (shown in percent, in parentheses next to each parameter).

\bye


==> paptable2.tex <==
\magnification=1200
\baselineskip=0.25truein
\hsize=16truecm
\vsize=22.5truecm
\topskip=1.5truecm
\nopagenumbers

\midinsert$$\vbox{\offinterlineskip
\halign{&\vrule#&\strut\ #\ \cr
\multispan{15}\hfil\bf Table II \hfil\cr
\hfil\cr
\noalign{\smallskip}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil $|V_{e2}|^2$\hfil&&\hfil $|V_{\mu 3}|^2$\hfil&&\hfil 
$|V_{e3}|^2$\hfil&&\hfil$\rho_1,\rho_2,|V_{\mu 1}|^2$\hfil&&\hfil
$cos(\delta)_-$\hfil&&\hfil $cos(\delta)_c$\hfil&&
\hfil $cos(\delta)_+$\hfil&\cr 
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.40 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
$\rho_1=0.68$ (5)\hfil&&\hfil -0.204\hfil&&
\hfil 0.025\hfil&&\hfil 0.247\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2=2.2$ (5)\hfil&&\hfil -0.294\hfil&&
\hfil -0.034\hfil&&\hfil 0.195\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$|V_{\mu 1}|^2=0.18$ (5)\hfil&&\hfil -0.615\hfil&&
\hfil -0.076\hfil&&\hfil 0.458\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (10)\hfil&&\hfil 0.40 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
$\rho_1=0.68$ (5)\hfil&&\hfil -0.213\hfil&&
\hfil 0.025\hfil&&\hfil 0.254\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil     \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$\rho_2=2.2$ (5)\hfil&&\hfil -0.446\hfil&&
\hfil -0.034\hfil&&\hfil 0.330\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.18$ (5)\hfil&&\hfil -0.813\hfil&&
\hfil -0.076\hfil&&\omit\hfil 0.665\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.40 (10)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
$\rho_1 = 0.68$ (5)\hfil&&\hfil -0.349\hfil&&
\hfil 0.025\hfil&&\omit\hfil 0.383\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$\rho_2=2.2$ (5)\hfil&&\hfil -0.310\hfil&&
\hfil -0.034\hfil&&\omit\hfil 0.199\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.18$ (5)\hfil&&\hfil -0.765\hfil&&
\hfil -0.076\hfil&&\omit\hfil 0.582\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.40 (5)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
$\rho_1 = 0.68$ (5)\hfil&&\hfil -0.212\hfil&&
\hfil 0.025\hfil&&\omit\hfil 0.250\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 2.2$ (5)\hfil&&\hfil -0.306\hfil&&
\hfil -0.034\hfil&&\omit\hfil 0.196\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.18$ (5)\hfil&&\hfil -0.628\hfil&&
\hfil -0.076\hfil&&\omit\hfil 0.471\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (2)\hfil&&\hfil 0.55 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
$\rho_1 = 0.8$ (2)\hfil&&\hfil 0.551\hfil&&
\hfil 0.650\hfil&&\omit\hfil 0.760\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 3.85$ (2)\hfil&&\hfil 0.541\hfil&&
\hfil 0.652\hfil&&\omit\hfil 0.770\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.145$ (2)\hfil&&\hfil 0.481\hfil&&
\hfil 0.663\hfil&&\omit\hfil 0.856\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (2)\hfil&&\hfil 0.55 (2)\hfil&&\hfil 0.01 (25) \hfil&&\hfil
$\rho_1 = 0.8$ (2)\hfil&&\hfil 0.553\hfil&&
\hfil 0.650\hfil&&\omit\hfil 0.854\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil    \hfil&&\hfil
$\rho_2 = 3.85$ (2)\hfil&&\hfil 0.543\hfil&&
\hfil 0.652\hfil&&\omit\hfil 0.852\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil    \hfil&&\hfil    \hfil&&\hfil     \hfil&&\hfil
$|V_{\mu 1}|^2=0.145$ (2)\hfil&&\hfil 0.482\hfil&&
\hfil 0.663\hfil&&\omit\hfil 0.993\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}\noalign{\smallskip}}}
$$\endinsert
\noindent
Values of $cos(\delta)$ for different 
combinations of parameters: $cos(\delta)_c$ is obtained  
from the central values of the parameters while $cos(\delta)_-$ and 
$cos(\delta)_+$ are the extremum values allowed by the 
uncertainties (shown in percent, in parentheses next to each parameter).

\bye


==> paptable3.tex <==
\magnification=1200
\baselineskip=0.25truein
\hsize=16truecm
\vsize=22.5truecm
\topskip=1.5truecm
\nopagenumbers

\midinsert$$\vbox{\offinterlineskip
\halign{&\vrule#&\strut\ #\ \cr
\multispan{13}\hfil\bf Table III \hfil\cr
\hfil\cr
\noalign{\smallskip}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil $|V_{e2}|^2$\hfil&&\hfil $|V_{\mu 3}|^2$\hfil&&\hfil 
$|V_{e3}|^2$\hfil&&\hfil
${|V_{\mu 1}|^2_-\atop |V_{\mu 1}|^2_+}$\hfil&&\hfil
$R_{e\mu}$\hfil&&\hfil $R_{e\tau}$\hfil&\cr 
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.3\hfil&&\hfil 0.5\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.11\atop 0.20}$\hfil&&\hfil ${0.94\atop 1.04}$\hfil&&
\hfil ${0.95\atop 1.06}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.3\hfil&&\hfil 0.5\hfil&&\hfil 0.005 \hfil&&\hfil
 ${0.12\atop 0.18}$\hfil&&\hfil ${0.96\atop 1.03}$\hfil&&
\hfil ${0.96\atop 1.03}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35\hfil&&\hfil 0.5\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.13\atop 0.23}$\hfil&&\hfil ${0.94\atop 1.03}$\hfil&&
\hfil ${0.96\atop 1.05}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35\hfil&&\hfil 0.55\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.12\atop 0.21}$\hfil&&\hfil ${0.88\atop 0.95}$\hfil&&
\hfil ${0.91\atop 0.99}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35\hfil&&\hfil 0.4\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.17\atop 0.26}$\hfil&&\hfil ${1.05\atop 1.14}$\hfil&&
\hfil ${1.14\atop 1.22}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35\hfil&&\hfil 0.6\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.10\atop 0.19}$\hfil&&\hfil ${0.80\atop 0.86}$\hfil&&
\hfil ${0.86\atop 0.95}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25\hfil&&\hfil 0.6\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.063\atop 0.145}$\hfil&&\hfil ${0.81\atop 0.90}$\hfil&&
\hfil ${0.86\atop 1.00}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.3\hfil&&\hfil 0.6\hfil&&\hfil 0.01 \hfil&&\hfil
 ${0.081\atop 0.17}$\hfil&&\hfil ${0.81\atop 0.88}$\hfil&&
\hfil ${0.86\atop 0.98}$\hfil&\cr
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
%\noalign{\hrule}
\noalign{\hrule}\noalign{\smallskip}}}
$$\endinsert


\noindent
Different values of $R_{e\mu}$ and $R_{e\tau}$ for different 
combinations of 4 independant $|V_{ij}|^2$. $|V_{\mu 1}|^2_-$ and 
$|V_{\mu 1}|^2_+$ span the range allowed by unitarity and positivity of 
$|J|^2$; these extremum values of $|V_{\mu 1}|^2$ correspond to vanishingly 
small CP-violation.


\bye


==> paptable4.tex <==
\magnification=1200
\baselineskip=0.25truein
\hsize=16truecm
\vsize=22.5truecm
\topskip=1.5truecm
\nopagenumbers

\midinsert$$\vbox{\offinterlineskip
\halign{&\vrule#&\strut\ #\ \cr
\multispan{15}\hfil\bf Table IV \hfil\cr
\hfil\cr
\noalign{\smallskip}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil $|V_{e2}|^2$\hfil&&\hfil $|V_{\mu 3}|^2$\hfil&&\hfil 
$|V_{e3}|^2$\hfil&&\hfil $R_{e\mu}$\hfil&&\hfil
$cos(\delta)_-$\hfil&&\hfil $cos(\delta)_c$\hfil&&
\hfil $cos(\delta)_+$\hfil&\cr 
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (1)\hfil&&\hfil 0.50 (1)\hfil&&\hfil 0.01 (1) \hfil&&\hfil
 1.00 (1)\hfil&&\hfil -0.183\hfil&&
\hfil 0.118\hfil&&\hfil 0.463\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (10)\hfil&&\hfil 0.5 (1)\hfil&&\hfil 0.01 (25) \hfil&&\hfil
 1.00 (1)\hfil&&\hfil -0.265\hfil&&
\hfil 0.118\hfil&&\hfil 0.567\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (2)\hfil&&\hfil 0.50 (2)\hfil&&\hfil 0.01 (2)\hfil&&\hfil
 1.00 (2)\hfil&&\hfil -0.463\hfil&&
\hfil 0.118\hfil&&\hfil 0.891\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (1)\hfil&&\hfil 0.50 (1)\hfil&&\hfil 0.005(1) \hfil&&\hfil
 1.00 (1)\hfil&&\hfil -0.332\hfil&&
\hfil 0.082\hfil&&\hfil 0.550\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (2)\hfil&&\hfil 0.50 (2)\hfil&&\hfil 0.005 (2) \hfil&&\hfil
 1.00 (2)\hfil&&\hfil -0.718\hfil&&
\hfil 0.082\hfil&&\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (1)\hfil&&\hfil 0.005 (10) \hfil&&\hfil
 1.00 (1)\hfil&&\hfil -0.373\hfil&&
\hfil 0.082\hfil&&\omit\hfil 0.600\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (1)\hfil&&\hfil 0.60 (1)\hfil&&\hfil 0.01 (1) \hfil&&\hfil
 0.84 (1)\hfil&&\hfil -0.605\hfil&&
\hfil -0.211\hfil&&\omit\hfil 0.257\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (2)\hfil&&\hfil 0.60 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 0.84 (2)\hfil&&\hfil -0.949\hfil&&
\hfil -0.211\hfil&&\omit\hfil 0.867\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.60 (1)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
 0.84 (1)\hfil&&\hfil -0.653\hfil&&
\hfil -0.211\hfil&&\omit\hfil 0.348\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35 (1)\hfil&&\hfil 0.45 (1)\hfil&&\hfil 0.01 (1) \hfil&&\hfil
 1.03 (1)\hfil&&\hfil -0.769\hfil&&
\hfil -0.485\hfil&&\omit\hfil -0.186\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35 (2)\hfil&&\hfil 0.45 (1)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 1.03 (1)\hfil&&\hfil -0.792\hfil&&
\hfil -0.485\hfil&&\omit\hfil -0.181\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35 (10)\hfil&&\hfil 0.45 (1)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
 1.03 (1)\hfil&&\hfil -0.931\hfil&&
\hfil -0.485\hfil&&\omit\hfil -0.121\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.35 (10)\hfil&&\hfil 0.45 (2)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
 1.03 (2)\hfil&&\hfil -0.936\hfil&&
\hfil -0.485\hfil&&\omit\hfil +0.160\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.24 (2)\hfil&&\hfil 0.40 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 1.06 (2)\hfil&&\hfil -0.476\hfil&&
\hfil -0.141\hfil&&\omit\hfil 0.205\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.24 (10)\hfil&&\hfil 0.40 (2)\hfil&&\hfil 0.01 (25) \hfil&&\hfil
 1.06 (2)\hfil&&\hfil -0.679\hfil&&
\hfil -0.141\hfil&&\omit\hfil 0.290\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.24 (2)\hfil&&\hfil 0.40 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 1.13 (2)\hfil&&\hfil 0.446\hfil&&
\hfil 0.845\hfil&&\omit\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.24 (10)\hfil&&\hfil 0.40 (1)\hfil&&\hfil 0.01 (25) \hfil&&\hfil
 1.13 (1)\hfil&&\hfil 0.579\hfil&&
\hfil 0.845\hfil&&\omit\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.24 (2)\hfil&&\hfil 0.40 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 1.13 (5)\hfil&&\hfil -0.076\hfil&&
\hfil 0.845\hfil&&\omit\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (1)\hfil&&\hfil 0.55 (1)\hfil&&\hfil 0.01 (1) \hfil&&\hfil
 0.94 (1)\hfil&&\hfil -0.165\hfil&&
\hfil 0.135\hfil&&\omit\hfil 0.475\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (10)\hfil&&\hfil 0.55 (1)\hfil&&\hfil 0.01 (25) \hfil&&\hfil
 0.94 (1)\hfil&&\hfil -0.244\hfil&&
\hfil 0.135\hfil&&\omit\hfil 0.627\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (2)\hfil&&\hfil 0.55 (2)\hfil&&\hfil 0.01 (2) \hfil&&\hfil
 0.94 (2)\hfil&&\hfil -0.440\hfil&&
\hfil 0.135\hfil&&\omit\hfil 0.874\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (5)\hfil&&\hfil 0.55 (2)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
 0.94 (2)\hfil&&\hfil -0.46\hfil&&
\hfil 0.135\hfil&&\omit\hfil 0.950\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
%\noalign{\hrule}
\noalign{\hrule}\noalign{\smallskip}}}
$$\endinsert
\noindent
Values of $cos(\delta)$ for different 
combinations of parameters: $cos(\delta)_c$ is obtained  
from the central values of the parameters while $cos(\delta)_-$ and 
$cos(\delta)_+$ are the extremum values allowed by the 
uncertainties (shown in percent, in parentheses next to each parameter).

\bye


==> paptable5.tex <==
\magnification=1200
\baselineskip=0.25truein
\hsize=16truecm
\vsize=22.5truecm
\topskip=1.5truecm
\nopagenumbers

\midinsert$$\vbox{\offinterlineskip
\halign{&\vrule#&\strut\ #\ \cr
\multispan{15}\hfil\bf Table V \hfil\cr
\hfil\cr
\noalign{\smallskip}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil $|V_{e2}|^2$\hfil&&\hfil $|V_{\mu 3}|^2$\hfil&&\hfil 
$|V_{e3}|^2$\hfil&&\hfil $\rho_1 = \phi^t_\tau/\phi^t_\mu$\hfil&&\hfil
$cos(\delta_{eff.})_-$\hfil&&\hfil $cos(\delta_{eff.})_c$\hfil&&
\hfil $cos(\delta_{eff.})_+$\hfil&\cr 
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 0.7 (5)\hfil&&\hfil 0.377\hfil&&
\hfil 0.628\hfil&&\hfil 0.920\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height5pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (10) \hfil&&\hfil
 0.7 (5)\hfil&&\hfil 0.378\hfil&&
\hfil 0.628\hfil&&\hfil 0.940\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5)\hfil&&\hfil
 0.7 (10)\hfil&&\hfil 0.303\hfil&&
\hfil 0.628\hfil&&\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (25)\hfil&&\hfil
 0.7 (5)\hfil&&\hfil 0.380\hfil&&
\hfil 0.628\hfil&&\hfil 1.0\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 1.3 (5)\hfil&&\hfil -0.685\hfil&&
\hfil -0.407\hfil&&\hfil -0.161\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 1.3 (10)\hfil&&\hfil -0.765\hfil&&
\hfil -0.407\hfil&&\hfil -0.072\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.30 (5)\hfil&&\hfil 0.50 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 1.8 (10)\hfil&&\hfil -1.0\hfil&&
\hfil -0.931\hfil&&\omit\hfil -0.598\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (5)\hfil&&\hfil 0.60 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 1.8 (5)\hfil&&\hfil -0.522\hfil&&
\hfil -0.263\hfil&&\omit\hfil -0.013\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (5)\hfil&&\hfil 0.60 (5)\hfil&&\hfil 0.01 (5) \hfil&&\hfil
 3.0 (10)\hfil&&\hfil -1.0\hfil&&
\hfil -0.920\hfil&&\omit\hfil -0.624\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
&\hfil 0.25 (5)\hfil&&\hfil 0.60 (5)\hfil&&\hfil 0.005 (5) \hfil&&\hfil
 2.5 (10)\hfil&&\hfil -1.0\hfil&&
\hfil -0.971\hfil&&\omit\hfil -0.544\hfil&\cr
height3pt&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&&\omit&\cr
\noalign{\hrule}
\noalign{\hrule}\noalign{\smallskip}}}
$$\endinsert
\noindent
Values of $cos(\delta_{eff.})$ for different 
combinations of parameters in a non-radiative decay scenario: 
$cos(\delta_{eff.})_c$ is obtained  
from the central values of the parameters while $cos(\delta_{eff.})_-$ and 
$cos(\delta_{eff.})_+$ are the extremum values allowed by the 
uncertainties (shown in percent, in parentheses next to each parameter).

\bye

